ATCN: Resource-Efficient Processing of Time Series on Edge

This paper presents a scalable deep learning model called Agile Temporal Convolutional Network (ATCN) for high-accurate fast classification and time series prediction in resource-constrained embedded systems. ATCN is a family of compact networks with formalized hyperparameters that enable application-specific adjustments to be made to the model architecture. It is primarily designed for embedded edge devices with very limited performance and memory, such as wearable biomedical devices and real-time reliability monitoring systems. ATCN makes fundamental improvements over the mainstream temporal convolutional neural networks, including residual connections to increase the network depth and accuracy, and the incorporation of separable depth-wise convolution to reduce the computational complexity of the model. As part of the present work, two ATCN families, namely T0, and T1 are also presented and evaluated on different ranges of embedded processors - Cortex-M7 and Cortex-A57 processor. An evaluation of the ATCN models against the best-in-class InceptionTime and MiniRocket shows that ATCN almost maintains accuracy while improving the execution time on a broad range of embedded and cyber-physical applications with demand for real-time processing on the embedded edge. At the same time, in contrast to existing solutions, ATCN is the first time-series classifier based on deep learning that can be run bare-metal on embedded microcontrollers (Cortex-M7) with limited computational performance and memory capacity while delivering state-of-the-art accuracy.

==> Tables/DeepRace_ExePerf.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Performance comparison of ATCN and LSTM (Deep RACE) running on Nvidia Tegra X1 (Jetson Nano)}
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}[2]{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Execusion Performance (mS)}} \\
          & \textbf{Average} & \textbf{Best} \\
    \midrule
    \textbf{ATCN} & 29.9  & 14.8 \\
    \textbf{LSTM} & 90.4  & 77 \\
    \textbf{Improvement} & 3.02$\times$  & 5.20$\times$ \\
    \bottomrule
    \end{tabular}%
  \label{tab:deepRace_performance}%
\end{table}%


==> Tables/UCR.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
	%\centering
%	\caption{Add caption}
	\begin{longtable}{lllllll}

		\caption{Description of 70 benchmarks selected from UCR Time Series Classification Archive 2018}\\
		\toprule
		\textbf{ID} & \textbf{Type} & \textbf{Name} & \textbf{Train} & \textbf{Test} & \textbf{Class} & \textbf{Length} \\
		\midrule
		\endfirsthead
		\multicolumn{4}{c}%
		{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
		\toprule
		\textbf{ID} & \textbf{Type} & \textbf{Name} & \textbf{Train} & \textbf{Test} & \textbf{Class} & \textbf{Length} \\
		\midrule
		\endhead
		\hline \multicolumn{4}{r}{\textit{Continued on next page}} \\
		\endfoot
		\hline
		\endlastfoot



		%\toprule
		%\textbf{ID} & \textbf{Type} & \textbf{Name} & \textbf{Train} & \textbf{Test} & \textbf{Class} & \textbf{Length} \\
		%\midrule


		1     & ECG   & ECGFiveDays & 23    & 861   & 2     & 136 \\
		2     & Sensor & Plane & 105   & 105   & 7     & 144 \\
		3     & Simulated & TwoPatterns & 1000  & 4000  & 4     & 128 \\
		4     & Sensor & Trace & 100   & 100   & 4     & 275 \\
		5     & Power & PowerCons & 180   & 180   & 2     & 144 \\
		6     & Spectro & Coffee & 28    & 28    & 2     & 286 \\
		7     & Simulated & BME   & 30    & 150   & 3     & 128 \\
		8     & Motion & GunPointMaleVersusFemale & 135   & 316   & 2     & 150 \\
		9     & Motion & GunPointOldVersusYoung & 136   & 315   & 2     & 150 \\
		10    & EPG   & InsectEPGRegularTrain & 62    & 249   & 3     & 601 \\
		11    & Sensor & Wafer & 1000  & 6164  & 2     & 152 \\
		12    & Simulated & SyntheticControl & 300   & 300   & 6     & 60 \\
		13    & Sensor & FreezerRegularTrain & 150   & 2850  & 2     & 301 \\
		14    & Traffic & Chinatown & 20    & 343   & 2     & 24 \\
		15    & Simulated & ShapeletSim & 20    & 180   & 2     & 500 \\
		16    & Motion & GunPointAgeSpan & 135   & 316   & 2     & 150 \\
		17    & ECG   & TwoLeadECG & 23    & 1139  & 2     & 82 \\
		18    & Motion & GunPoint & 50    & 150   & 2     & 150 \\
		19    & Simulated & UMD   & 36    & 144   & 3     & 150 \\
		20    & Sensor & DodgerLoopWeekend & 20    & 138   & 2     & 288 \\
		21    & Device & HouseTwenty & 40    & 119   & 2     & 2000 \\
		22    & Motion & ToeSegmentation2 & 36    & 130   & 2     & 343 \\
		23    & Sensor & ItalyPowerDemand & 67    & 1029  & 2     & 24 \\
		24    & Simulated & CBF   & 30    & 900   & 3     & 128 \\
		25    & Image & Symbols & 25    & 995   & 6     & 398 \\
		26    & Sensor & FordA & 3601  & 1320  & 2     & 500 \\
		27    & Image & Fish  & 175   & 175   & 7     & 463 \\
		28    & Image & DiatomSizeReduction & 16    & 306   & 4     & 345 \\
		29    & ECG   & ECG5000 & 500   & 4500  & 5     & 140 \\
		30    & ECG   & ECG200 & 100   & 100   & 2     & 96 \\
		31    & Motion & ToeSegmentation1 & 40    & 228   & 2     & 277 \\
		32    & Spectro & Strawberry & 613   & 370   & 2     & 235 \\
		33    & Sensor & SonyAIBORobotSurface1 & 20    & 601   & 2     & 70 \\
		34    & Sensor & FreezerSmallTrain & 28    & 2850  & 2     & 301 \\
		35    & Image & MixedShapesRegularTrain & 500   & 2425  & 5     & 1024 \\
		36    & Sensor & DodgerLoopGame & 20    & 138   & 2     & 288 \\
		37    & Spectrum & SemgHandGenderCh2 & 300   & 600   & 2     & 1500 \\
		38    & Image & BirdChicken & 20    & 20    & 2     & 512 \\
		39    & Sensor & SonyAIBORobotSurface2 & 27    & 953   & 2     & 65 \\
		40    & Sensor & Lightning2 & 60    & 61    & 2     & 637 \\
		41    & Image & ProximalPhalanxOutlineCorrect & 600   & 291   & 2     & 80 \\
		42    & Image & ProximalPhalanxOutlineAgeGroup & 400   & 205   & 3     & 80 \\
		43    & Device & LargeKitchenAppliances & 375   & 375   & 3     & 720 \\
		44    & Sensor & Car   & 60    & 60    & 4     & 577 \\
		45    & Sensor & MoteStrain & 20    & 1252  & 2     & 84 \\
		46    & Sensor & FordB & 3636  & 810   & 2     & 500 \\
		47    & Image & ArrowHead & 36    & 175   & 3     & 251 \\
		48    & Image & BeetleFly & 20    & 20    & 2     & 512 \\
		49    & Image & ProximalPhalanxTW & 400   & 205   & 6     & 80 \\
		50    & Device & SmallKitchenAppliances & 375   & 375   & 3     & 720 \\
		51    & Image & FaceAll & 560   & 1690  & 14    & 131 \\
		52    & Motion & UWaveGestureLibraryX & 896   & 3582  & 8     & 315 \\
		53    & Spectrum & SemgHandSubjectCh2 & 450   & 450   & 5     & 1500 \\
		54    & Image & DistalPhalanxOutlineAgeGroup & 400   & 139   & 3     & 80 \\
		55    & Sensor & Earthquakes & 322   & 139   & 2     & 512 \\
		56    & Motion & WormsTwoClass & 181   & 77    & 2     & 900 \\
		57    & Sensor & Lightning7 & 70    & 73    & 7     & 319 \\
		58    & Spectro & Ham   & 109   & 105   & 2     & 431 \\
		59    & Image & DistalPhalanxTW & 400   & 139   & 6     & 80 \\
		60    & Motion & UWaveGestureLibraryZ & 896   & 3582  & 8     & 315 \\
		61    & Device & Computers & 250   & 250   & 2     & 720 \\
		62    & Device & ElectricDevices & 8926  & 7711  & 7     & 96 \\
		63    & Motion & UWaveGestureLibraryY & 896   & 3582  & 8     & 315 \\
		64    & Sensor & InsectWingbeatSound & 220   & 1980  & 11    & 256 \\
		65    & Image & MiddlePhalanxOutlineAgeGroup & 400   & 154   & 3     & 80 \\
		66    & Image & Herring & 64    & 64    & 2     & 512 \\
		67    & Image & MiddlePhalanxTW & 399   & 154   & 6     & 80 \\
		68    & EOG   & EOGVerticalSignal & 362   & 362   & 12    & 1250 \\
		69    & Sensor & DodgerLoopDay & 78    & 80    & 7     & 288 \\
		70    & Device & RefrigerationDevices & 375   & 375   & 3     & 720 \\
%		\bottomrule
    \label{tab:ucr_db}%
\end{longtable}%
	
%\end{table}%


==> Tables/avg_accuracy.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
  \centering
  \caption{Comparison of the average accuracy for seventy benchmarks from the 2018 UCR time series classification dataset}
    \begin{tabular}{lcccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Metric}}} & \multicolumn{4}{c}{\textbf{Models}} \\
\cmidrule{2-5}          & \multicolumn{1}{c}{\textbf{T0}} & \multicolumn{1}{c}{\textbf{T1}} & \multicolumn{1}{c}{\textbf{T2}} & \multicolumn{1}{c}{\textbf{InceptionTime}} \\
    \midrule
    \textbf{Average Accuracy} & 83.69\% & 85.73\% & 86.65\% & 86.28\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:avg_acc}%
\end{table}%


==> Tables/ecg_arch.tex <==
% Table generated by Excel2LaTeX from sheet 'Network'
\begin{table}[htbp]
  \centering
  \caption{ATCN network architecture for heartbeat classification}
%        \begin{adjustbox}{width=1.\linewidth,center}

    \begin{tabular}{cccc}
    \toprule
    \textbf{Block type} & Kernel size ($k$) & Dilation Size ($d$) &  Output channel size ($c_{in})$ \\
    \midrule
    RCB   & 24    & 1     & 320 \\
    LCB   & 16    & 2     & 256 \\
    LCB   & 16    & 4     & 256 \\
    LCB   & 16    & 4     & 256 \\
    LCB   & 16    & 4     & 256 \\
    STCB  & 8     & 4     & 128 \\
    LCB   & 8     & 6     & 128 \\
    LCB   & 8     & 6     & 128 \\
    LCB   & 8     & 6     & 128 \\
    LCB   & 8     & 6     & 128 \\
    STCB  & 8     & 8     & 64 \\
    LCB   & 8     & 8     & 64 \\
    LCB   & 8     & 8     & 64 \\
    Average Pooling & -     & -     & 64 \\
    Linear & -     & -     & 3 \\
    \bottomrule
    \end{tabular}%
%    \end{adjustbox}
  \label{tab:ecg_arch}%
\end{table}%


==> Tables/ecg_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
  \centering
  \caption{ECG - Performance results comparison}
 %     \begin{adjustbox}{width=1.0\linewidth,center}

    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[4]{*}{} & \multirow{2}[4]{*}{\textbf{Input size}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Params(M)}}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Ops(G)}}} & \multicolumn{4}{c}{\textbf{F1}} & \multirow{2}[4]{*}{\textbf{Accuracy}} \\
\cmidrule{5-8}          &       &       &       & \textbf{N} & \textbf{A} & \textbf{O} & \textbf{AVG} &  \\
    \midrule
    \textbf{ATCN} & 18000 & 1.80  & 14.70 & 0.94  & 0.79  & 0.89  & 0.88  & 0.91 \\
    \textbf{DeepECG} & 18000 & 5.39  & 45.49 & 0.92  & 0.81  & 0.80  & 0.84  & 0.88 \\
    \textbf{Improvement} & -     & 2.99$\times$  & 3.09$\times$  & 0.02  & -0.02 & 0.09  & 0.04  & 0.03 \\
    \bottomrule
    \end{tabular}%
%    \end{adjustbox}
  \label{tab:ecg}%
\end{table*}%


==> Tables/mnist.tex <==
% Table generated by Excel2LaTeX from sheet 'MNIST'
\begin{table}[htbp]
  \centering
  \caption{MNIST - Performance results comparison}
%  \begin{adjustbox}{width=0.75\linewidth,center}
    \begin{tabular}{cccc}
    \toprule
          & \textbf{Accuracy} & \textbf{Parameters\newline{}(K)} & \textbf{Ops \newline{}(M)} \\
    \midrule
    \textbf{ATCN} & 0.99  & 8.47  & 3.98 \\
    \textbf{GTCN} & 0.99  & 66.91 & 65.85 \\
    \textbf{Improvement} & 0 & 7.90$\times$  & 16.56$\times$ \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
 %   \end{adjustbox}
  \label{tab:mnsit_res}%
\end{table}%

==> Tables/mnist_arch.tex <==
% Table generated by Excel2LaTeX from sheet 'Network'
\begin{table}[htbp]
  \centering
  \caption{ATCN network architecture for MNIST classification}
%    \begin{adjustbox}{width=1.\linewidth,center}

    \begin{tabular}{cccc}
    \toprule
    \textbf{Block type} & Kernel size ($k$) & Dilation Size ($d$) &  Output channel size ($c_{in})$ \\
    \midrule
    RCB   & 25     & 1     & 8 \\
    LCB   & 13    & 2     & 16 \\
    LCB   & 13    & 2     & 16 \\
    STCB   & 7    & 4     & 24 \\
    LCB   & 7    & 4     & 24 \\
    STCB   & 5    & 6     & 32 \\
    LCB   & 5    & 6     & 32 \\
    Average Pooling & -     & -     & 32 \\
    Linear & -     & -     & 10 \\
    \bottomrule
    \end{tabular}%
 %   \end{adjustbox}
  \label{tab:mnist_arch}%
\end{table}%

==> Tables/mosfet_arch.tex <==
% Table generated by Excel2LaTeX from sheet 'Network'
\begin{table}[htbp]
  \centering
  \caption{ATCN network architecture for MOSFET degradation modeling}
 %\begin{adjustbox}{width=1.\linewidth,center}
    \begin{tabular}{cccc}
    \toprule
    \textbf{Block type} & Kernel size ($k$) & Dilation Size ($d$) &  Output channel size ($c_{in}$) \\
    \midrule
    RCB   & 11    & 1     & 8 \\
    LCB   & 5    & 2     & 16 \\
    LCB   & 5    & 2     & 16 \\
    LCB   & 3    & 4     & 32 \\
    Linear & -     & -   & 104 \\
    \bottomrule
    \end{tabular}%
 %   \end{adjustbox}
  \label{tab:mosfet_arch}%
\end{table}%


==> Tables/mosfet_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
  \centering
  \caption{Performance results comparison}
  %    \begin{adjustbox}{width=1.\linewidth,center}

    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[4]{*}{} & \multirow{2}[4]{*}{\textbf{Input size}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Model Size (K)}}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Operations (K)\newline{}}}} & \multicolumn{5}{c}{\textbf{Log(MSE)}} \\
\cmidrule{5-9}          &       &       &       & \textbf{8} & \textbf{9} & \textbf{14} & \textbf{36} & \textbf{AVG}  \\
    \midrule
    \textbf{ATCN} & 21          & 7.67    & 103.5  & -6.26  & -6.33  & -5.62  & -6.18  & -5.99  \\
    \textbf{Deep RACE} & 21          & 32.74   & 64.47  & -6.16  & -5.71  & -5.61  & -6.16  & -5.84 \\
    \textbf{Improvement} & -    & 4.27$\times$   &-33.77\%  & -20.24\%   & -76.12\%  & -3.15\%  & -4.52\%    & -29.94\% \\
    \bottomrule
    \end{tabular}%
 %   \end{adjustbox}
  \label{tab:mosfet_result}%
\end{table*}%


==> Tex/Acknowledgment.tex <==
\begin{acks}
This work was supported by the National Science Foundation (NSF) under Award No. 1831795.
\end{acks}
